Black-box $\alpha$-divergence Minimization

Black-box alpha (BB-$\alpha$) is a new approximate inference method based on the minimization of $\alpha$-divergences. BB-$\alpha$ scales to large datasets because it can be implemented using stochastic gradient descent. BB-$\alpha$ can be applied to complex probabilistic models with little effort since it only requires as input the likelihood function and its gradients. These gradients can be easily obtained using automatic differentiation. By changing the divergence parameter $\alpha$, the method is able to interpolate between variational Bayes (VB) ($\alpha \rightarrow 0$) and an algorithm similar to expectation propagation (EP) ($\alpha = 1$). Experiments on probit regression and neural network regression and classification problems show that BB-$\alpha$ with non-standard settings of $\alpha$, such as $\alpha = 0.5$, usually produces better predictions than with $\alpha \rightarrow 0$ (VB) or $\alpha = 1$ (EP).

==> tables/mnist_table.tex <==
\begin{table*}[!ht]
\centering
\caption{Average Test Error and Test Log-likelihood in MNIST.}
\begin{tabular}{l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}}\hline
{\bf MNIST Dataset} &\multicolumn{2}{c}{\bf{ BB-$\alpha{=}1.0$ }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}0.5$ }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}10^{-6}$ }}&\multicolumn{2}{c}{\bf{ BB-VB }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}-1.0$ }}\\
\hline
\bf{Avg. Error} &0.0151&0.0001&0.0144&0.0001&0.0136&0.0001&0.0136&0.0001&\bf{0.0133}&\bf{0.0001}\\
\bf{Avg. Rank} &  4.975  &  0.025 &  4.025  &  0.025 &  2.150  &  0.115 &  2.125  &  0.153 &  {\bf 1.725 } &  {\bf 0.210}\\
\hline
\bf {Avg. Log-likelihood} &-0.0551&0.0004&-0.0509&0.0003&-0.0468&0.0002&-0.0468&0.0002&\bf{-0.0447}&\bf{0.0002}\\
\bf{Avg. Rank} &  5.0000  &  0.0000 &  4.0000  &  0.0000 &  2.5500  &  0.1141 &  2.4500  &  0.1141 &  {\bf 1.0000}  &  {\bf 0.0000}\\
\hline
\end{tabular}
\label{tab:results_mnist}
\end{table*}


==> tables/table_probit_error.tex <==
\begin{table*}[!ht]
\centering
\caption{ Average Test Error Probit Regression. }
%\resizebox{\columnwidth}{!}{
\begin{tabular}{l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}}\hline
\bf{Dataset}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}1.0$ }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}0.5$ }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}10^{-6}$ }}&\multicolumn{2}{c}{\bf{ BB-VB }}\\
\hline
Ionosphere&0.124&0.008&0.124&0.008&\bf{0.123}&\bf{0.008}&0.123&0.008\\
Madelon&\bf{0.445}&\bf{0.005}&0.454&0.005&0.457&0.005&0.457&0.005\\
Pima&\bf{0.234}&\bf{0.006}&0.234&0.006&0.235&0.006&0.235&0.006\\
Colon&\bf{0.303}&\bf{0.028}&0.307&0.028&0.307&0.028&0.307&0.028\\
\hline
\bf{Avg. Rank} &  2.322  &  0.048 &  2.513  &  0.039 &  2.587  &  0.031 &  2.578  &  0.031\\
\hline
\end{tabular}
\label{tab:results_probit_regression_error}
%}
\end{table*}


==> tables/table_probit_ll.tex <==
\begin{table*}[!ht]
\centering
\caption{ Average Test Log-likelihood Probit Regression.}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}r@{$\pm$}l@{\ica}}\hline
\bf{Dataset}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}1.0$ }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}0.5$ }}&\multicolumn{2}{c}{\bf{ BB-$\alpha{=}10^{-6}$ }}&\multicolumn{2}{c}{\bf{ BB-VB }}\\
\hline
Ionosphere&-0.3329&0.0218&-0.3328&0.0218&-0.3327&0.0217&\bf{-0.3327}&\bf{0.0217}\\
Madelon&\bf{-0.7991}&\bf{0.0057}&-0.9197&0.0084&-0.9534&0.0092&-0.9534&0.0092\\
Pima&\bf{-0.5007}&\bf{0.0102}&-0.5009&0.0102&-0.5012&0.0102&-0.5012&0.0102\\
Colon Cancer&\bf{-2.2608}&\bf{0.4062}&-2.2637&0.4068&-2.2684&0.4076&-2.2684&0.4076\\
\hline
\bf{Avg. Rank} &  1.8950  &  0.0970 &  2.2900  &  0.0379 &  2.9700  &  0.0730 &  2.8450  &  0.0720\\
\hline
\end{tabular}
\label{tab:results_probit_regression_ll}
%}
\end{table*}


